Bias in the representative volume element method: periodize the ensemble instead of its realizations

We study the Representative Volume Element (RVE) method, which is a method to approximately infer the effective behavior $a_{\text{hom}}$ of a stationary random medium. The latter is described by a coefficient field $a(x)$ generated from a given ensemble $\langle\cdot\rangle$ and the corresponding linear elliptic operator $-\nabla\cdot a\nabla$. In line with the theory of homogenization, the method proceeds by computing $d = 3$ correctors (d denoting the space dimension).To be numerically tractable, this computation has to be done on a finite domain: the so-called "representative" volume element, i. e. a large box with, say, periodic boundary conditions. The main message of this article is: Periodize the ensemble instead of its realizations. By this we mean that it is better to sample from a suitably periodized ensemble than to periodically extend the restriction of a realization $a(x)$ from the whole-space ensemble $\langle\cdot\rangle$. We make this point by investigating the bias (or systematic error), i. e. the difference between $a_{\text{hom}}$ and the expected value of the RVE method, in terms of its scaling w. r. t. the lateral size $L$ of the box. In case of periodizing $a(x)$, we heuristically argue that this error is generically $O(L^{-1})$. In case of a suitable periodization of $\langle\cdot\rangle$, we rigorously show that it is $O(L^{-d})$. In fact, we give a characterization of the leading-order error term for both strategies, and argue that even in the isotropic case it is generically non-degenerate. We carry out the rigorous analysis in the convenient setting of ensembles $\langle\cdot\rangle$ of Gaussian type with integrable covariance, which allow for a straightforward periodization and which make the Price theorem and the Malliavin calculus available for optimal stochastic estimates of correctors.

==> Commandes.tex <==
%%%Ensembles
\newcommand{\R}{\mathbb{R}}
\newcommand{\C}{\mathbb{C}}
\newcommand{\Z}{\mathbb{Z}} 
\newcommand{\QQ}{\mathcal{Q}}
\newcommand{\NN}{\mathbb{N}}

%% Espaces fonctionnels
\newcommand{\LL}{{\rm{L}}}
\newcommand{\CC}{{\rm{C}}}
\newcommand{\HH}{{\rm{H}}}
\newcommand{\WW}{{\rm{W}}}
\newcommand{\LLinf}{\LL^\infty(\R)}
\newcommand{\WWinf}{\WW^{1,\infty}(\R)}
\newcommand{\Lunif}{\LL_{\rm unif}}
\newcommand{\BMO}{{\rm BMO}}
\newcommand{\Besov}{{\rm B}}

%%droite/gauche, parenthèses
\newcommand{\lt}{\left}
\newcommand{\rt}{\right}
\def\[{[\![}
\def\]{]\!]}

%opérateurs en lettres droites
\newcommand{\sgn}{{\rm{sign}}}
\newcommand{\dd}{{\rm d}}
\newcommand{\im}{{\rm{i}}}
\newcommand{\Supp}{{\rm{Supp}}}
\newcommand{\pv}{{\rm{p.v.}}}
\newcommand{\ee}{{\rm{e}}}
\newcommand{\ii}{{\rm{i}}}
\newcommand{\Id}{{\rm Id}}
\newcommand{\un}{\textbf{1}}
\newcommand{\esssup}{{\rm{ess~sup}}}
\newcommand{\essinf}{{\rm{ess~inf}}}

\renewcommand{\div}{{\rm div}}
\renewcommand{\Re}{{\rm Re\,}}
\renewcommand{\Im}{{\rm Im\,}}
\newcommand{\argmin}{{\rm{arg\,min}}}
\newcommand{\argmax}{{\rm{arg\,max}}}

%% Transformations
\newcommand{\FF}{\mathcal{F}}
\newcommand{\Hilb}{\mathcal{H}}
\newcommand{\Lap}{\mathcal{L}}

%%%underset importants
\newcommand{\loc}{{\rm{loc}}}
\newcommand{\comp}{{\rm{c}}}
\newcommand{\per}{{\rm per}}
\newcommand{\unif}{{\rm unif}}

%%%%%%%%%%%%%%%%%%%%%%%% Notations spéciales
\newcommand{\dx}{\lt|\partial_x\rt|}

%%%%%%%%%%%%%%%%%%%%%%%%underline/overline
\newcommand{\ov}{\overline}
\newcommand{\und}{\underline}

%%%%%%%%%%%%%%%%%%%%%%%% symboles logiques
\newcommand{\rtar}{\rightarrow}
\newcommand{\Rtar}{\Longrightarrow}
\newcommand{\rtarl}{\longritharrow}
\newcommand{\rthp}{\rightharpoonup}

%%%%%%%%%%%%%%%%%%%%%%%% couleurs
\newcommand{\red}{\color{red}}
\newcommand{\redforme}{\color{red} Rk \affichecompt [for Marc]}
\newcommand{\blue}{\color{blue}  Rk \affichecompt:}
\newcommand{\affichecompt}{\addtocounter{Compteur}{1} \arabic{Compteur}}

%%%%%%%%%%%%%%%%%%%%%%%% Ensembles géométriques
\newcommand{\Boule}{{\rm B}}
\newcommand{\Q}{{\rm Q}}
\newcommand{\dist}{{\rm d}}

%%%%%%%%%%%%%%%%%%%%%%%% Integrales
\def\fint{\dashint}


%%%%%%%%%%%% epsilon
\renewcommand{\epsilon}{\varepsilon}
\renewcommand{\tilde}{\widetilde}
\newcommand{\langl}{\lt\langle}
\newcommand{\rangl}{\rt\rangle}

\newcommand{\Torus}{\mathbb{T}}

\newcommand{\mvdots}{{\footnotesize \smash{\vdots}}}

==> CommandesANG.tex <==
%%%%%%%%%%%%%%%%%%%%%%%% connecteurs équation
\newcommand{\et}{\;\;\;\;\text{and}\;\;\;}
\newcommand{\dans}{\;\;\;\;\text{in}\;\;\;\;}
\newcommand{\si}{\;\;\;\;\text{if}\;\;\;\;}
\newcommand{\ou}{\;\;\;\;\text{or}\;\;\;\;}
\newcommand{\pour}{\;\;\;\;\text{for}\;\;\;\;}
\newcommand{\pourtout}{\;\;\;\;\text{for all}\;}
\newcommand{\sur}{\;\;\;\;\text{on}\;}

==> Commandes_adhoc.tex <==
\newcommand{\Dom}{{\rm D}}
\newcommand{\Interf}{\mathcal{I}}

\newcommand{\Sigpot}{\sigma}
\newcommand{\GDelta}{\mathcal{G}_\Delta}

%%%% Coord \abar-harmoniques
\newcommand{\nablabar}{\bar{\nabla}}
\newcommand{\partialbar}{\bar{\partial}}
\renewcommand{\P}{P}

%%%% phi
\newcommand{\wdef}{\widetilde{\phi}}
\newcommand{\wper}{\phi^{\rm per}}

%%%% u
\newcommand{\ueps}{u^\epsilon}
\newcommand{\ubar}{\bar{u}}
\newcommand{\vbar}{\bar{v}}
\newcommand{\uper}{u^\per}
\newcommand{\utilde}{\widetilde{u}}
\newcommand{\UUU}{\bar{\nabla}u}

%%%% a
\newcommand{\aper}{a_{\rm per}}
\newcommand{\adef}{\widetilde{a}}
\newcommand{\aeps}{a_\epsilon}
\newcommand{\abar}{\bar{a}}



%%%% reste
\newcommand{\Reste}{R}
\newcommand{\Reps}{\Reste^\epsilon}

%%%% Excess
\newcommand{\Exc}{\mathcal{E}}
\newcommand{\rstar}{r_*}
\newcommand{\rmax}{r_{\max}}


%%%% chapeaux
\newcommand{\vecphi}{\check{\phi}}
\newcommand{\vecsigma}{\check{\sigma}}
\newcommand{\s}{\tilde{\sigma}}
\newcommand{\w}{\tilde{\phi}}
\newcommand{\vecdelta}{\check{\delta}}


%%%% Q
\newcommand{\Ring}{{\rm R}}
\newcommand{\QU}{\mathcal{Q}}

\newcommand{\barC}{\bar{C}}

\newcommand{\fff}{g}
\newcommand{\gggg}{f}

\newcommand{\nuuu}{q}
